Supervised brain node and network construction under voxel-level functional imaging

Recent advancements in understanding the brain's functional organization related to behavior have been pivotal, particularly in the development of predictive models based on brain connectivity. Traditional methods in this domain often involve a two-step process by first constructing a connectivity matrix from predefined brain regions, and then linking these connections to behaviors or clinical outcomes. However, these approaches with unsupervised node partitions predict outcomes inefficiently with independently established connectivity. In this paper, we introduce the Supervised Brain Parcellation (SBP), a brain node parcellation scheme informed by the downstream predictive task. With voxel-level functional time courses generated under resting-state or cognitive tasks as input, our approach clusters voxels into nodes in a manner that maximizes the correlation between inter-node connections and the behavioral outcome, while also accommodating intra-node homogeneity. We rigorously evaluate the SBP approach using resting-state and task-based fMRI data from both the Adolescent Brain Cognitive Development (ABCD) study and the Human Connectome Project (HCP). Our analyses show that SBP significantly improves out-of-sample connectome-based predictive performance compared to conventional step-wise methods under various brain atlases. This advancement holds promise for enhancing our understanding of brain functional architectures with behavior and establishing more informative network neuromarkers for clinical applications.

==> results/ABCD-HCP-combined.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!htb]
\centering
\caption{Performance comparison for HCP and ABCD data. The average out of sample $R^2$ from 10 folds is reported in the table.} %\yize{add another row--proposed methods/existing ones. Also keep the digital number the same}}
\label{tab:r2-abcd-hcp}
% \resizebox{.8\textwidth}{!}{%
% % \usepackage{tabularray}
% \usepackage{tabularray}
% \begin{table}
% \centering
\begin{tblr}{
vspan=even,
  cells = {c},
  cell{1}{1} = {r=2}{r},
  cell{1}{2} = {r=2}{},
  cell{1}{3} = {c=3}{},
  cell{1}{6} = {c=3}{},
  cell{3}{1} = {c=2}{},
  cell{4}{1} = {r},
  cell{5}{1} = {r},
  cell{6}{1} = {r},
  cell{7}{1} = {r},
  cell{8}{1} = {r},
  cell{9}{1} = {c=2}{},
  cell{10}{1} = {r},
  cell{11}{1} = {r},
  cell{12}{1} = {r},
  cell{13}{1} = {r},
  vline{3} = {1-2}{},
  vline{4} = {1}{},
  vline{6} = {1-2}{},
  vline{3,6} = {4-8,10-13}{},
  hline{1,14} = {-}{0.2em},
  hline{2} = {3-8}{},
  hline{3-4,9-10} = {-}{}
}
Atlas                    & \# Regions & ABCD           &                &                & HCP            &                &                \\
                         &            & Rest           & MID            & nBack          & Rest           & Language       & Emotion        \\
\textit{Proposed method} &            &                &                &                &                &                &                \\
SBP                      & 100        & 0.064          & 0.086          & 0.078          & 0.025          & 0.117          & 0.109          \\
SBP                      & 200        & 0.075          & 0.105          & 0.094          & 0.038          & 0.124          & 0.119          \\
SBP                      & 300        & 0.088          & 0.106          & 0.103          & 0.042          & 0.132          & 0.131          \\
SBP                      & 400        & 0.092          & 0.108          & \textbf{0.107} & \textbf{0.044} & \textbf{0.137} & \textbf{0.133} \\
SBP                      & 500        & \textbf{0.095} & \textbf{0.112} & 0.103          & 0.042          & 0.135          & 0.129          \\
\textit{Existing atlas}  &            &                &                &                &                &                &                \\
AAL3                     & 170        & 0.004          & 0.055          & 0.045          & 0.005          & 0.072          & 0.066          \\
Shen268                  & 268        & 0.008          & 0.072          & 0.066          & 0.012          & 0.106          & 0.093          \\
Shen368                  & 368        & 0.004          & 0.082          & 0.057          & 0.037          & 0.115          & 0.106          \\
Schaefer                 & 400        & 0.005          & 0.077          & 0.059          & 0.029          & 0.112          & 0.107          
\end{tblr}
\end{table}

==> results/abcd-connectivity.tex <==
\begin{figure}[H]
    \centering
     \begin{subfigure}[b]{0.75\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/ABCD-rest-connectivity.png}
         \caption{SEK-400 (Rest)}
     \end{subfigure}
     
     \vfill
     \begin{subfigure}[b]{0.75\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/ABCD-rest-connectivity.png}
         \caption{SEK-400 (MID)}
     \end{subfigure}
     
     \vfill
     \begin{subfigure}[b]{0.75\textwidth}
         \centering
        \includegraphics[width=\textwidth]{imgs/ABCD-rest-connectivity.png}
         \caption{SEK-400 (nBack)}
     \end{subfigure}

    \caption{Whole brain parcellation plots visualized with BioImage Suite on ABCD.}
    \label{fig:abcd-connectivity}
\end{figure}





==> results/abcd-cpm.tex <==
\begin{figure}[H]
    \centering
     \begin{subfigure}[t]{0.25\textwidth}
         \centering
         % \includegraphics[width=0.256\textwidth]{imgs/ABCD-actual-predicted-Rest.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-positive-Rest.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-negative-Rest.png}
         \caption{Rest}
     \end{subfigure}
     %\hfill
      \begin{subfigure}[t]{0.25\textwidth}
         \centering
         % \includegraphics[width=0.256\textwidth]{imgs/ABCD-actual-predicted-MID.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-positive-MID.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-negative-MID.png}
         \caption{MID}
     \end{subfigure}     
     %\hfill
      \begin{subfigure}[t]{0.25\textwidth}
         \centering
         % \includegraphics[width=0.256\textwidth]{imgs/ABCD-actual-predicted-nBack.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-positive-nBack.png}
         \includegraphics[width=0.99\textwidth]{imgs/ABCD-heatmap-negative-nBack.png}
         \caption{nBack}
     \end{subfigure}
     % \vfill
     % \begin{subfigure}{0.85\textwidth}
     %     \centering
     %     \includegraphics[width=0.99\textwidth]{imgs/fn-legend.png}
     %     %\caption{nBack}
     % \end{subfigure}
    \caption{Heatmap of the top $20\%$ selected edges with the highest absolute value of coefficient from CPM based on SEC(400) parcellation with ABCD data. The top row and bottom row visualized the positive and negative edges, and the left, middle and right column corresponds to Rest, MID and nBack respectively. The functional networks in the plots corresponds to: 1. medial frontal, 2. fronto parietal, 3. default mode, 4. motor, 5. visual I, 6. visual II, 7. visual association, 8. limbic,  9. basal ganglia, and 10. cerebellum. }
    \label{fig:abcd-cpm-plots}
\end{figure}




==> results/abcd-hcp-glassbrain.tex <==
\begin{figure}[H]
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width = 1\textwidth]{imgs/ABCD-rsfMRI-glassbrain.png}
         \includegraphics[width = 1\textwidth]{imgs/ABCD-MID-glassbrain.png}
         \includegraphics[width = 1\textwidth]{imgs/ABCD-nBack-glassbrain.png}
         \caption{ABCD}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width = 1\textwidth]{imgs/HCP-REST2-glassbrain.png}
         \includegraphics[width = 1\textwidth]{imgs/HCP-LANGUAGE-glassbrain.png}
         \includegraphics[width = 1\textwidth]{imgs/HCP-EMOTION-glassbrain.png}
         \caption{HCP}
     \end{subfigure}
    \caption{Significant edges from the SEC(400) atlas was mapped to Shen268 atlas, and plotted on the glass brain. Blue/red lines indicate negative/positive correlation with the cognitive outcome, and the size of the node is proportion to the number of edges connecting that node. Left column is generated from the ABCD data, and the right column is generated from the HCP data. Each subfigure corresponds to the orthogonal coronal, sagittal and axial slices for each state. }
    \label{fig:abcd-hcp-glassbrain}
\end{figure}


==> results/abcd-parcellation-plots.tex <==
% \begin{figure}[H]
%     \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{\textcolor{black}{SEK-200 (Rest)}}
%      \end{subfigure}
%      \vfill
          
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{\textcolor{black}{SEK-200 (MID)}}
%      \end{subfigure}
%      \vfill
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{\textcolor{black}{SEK-200 (Language)}}
%      \end{subfigure}    
%      \vfill 
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \includegraphics[width=.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{SEK-400 (Rest)}
%      \end{subfigure}
%      \vfill
          
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{SEK-400 (MID)}
%      \end{subfigure}
%      \vfill
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/abcd-SEK-rest.png}
%          \caption{SEK-400 (Language)}
%      \end{subfigure}    

%     \caption{Whole brain parcellation plots visualized with BioImage Suite on ABCD.}
%     \label{fig:abcd-parcellation-plots}
% \end{figure}


\begin{table}[!ht]
  \centering
  \begin{tabular}{  m{1cm} | c | c }
    \hline
    \hline
     & SBP(200) & SBP(400) \\
    %SEK & Task & Parcellation 
    \hline
    Rest 
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC200-ABCD-rest.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-rest.png}
    \end{minipage}
    \\ \hline
    MID
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC200-ABCD-MID.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-MID.png}
    \end{minipage}
    \\ \hline
    nBack 
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC200-ABCD-nBack.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-nBack.png}
    \end{minipage}
    \\ \hline
    \hline
  \end{tabular}
  \caption{Brain maps generated with SBP(200) and SBP(400) based on ABCD dataset.}\label{tab:abcd-parc-plots}
\end{table}


==> results/abcd-sek400-ringplots.tex <==
\begin{figure}[H]
% rest
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-a}
    \caption{Rest - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{example-image-a}
    \caption{Rest Negative}
  \end{subfigure}   
  \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-abcd-rest.png}
        \caption{Rest 3d Brain}
  \end{subfigure}
  \vfill
%MID
\begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-a}
    \caption{MID - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{example-image-a}
    \caption{MID Negative}
  \end{subfigure}   
\begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-abcd-MID.png}
        \caption{Rest 3d Brain}
  \end{subfigure}
  \vfill
%NBACK
\begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-a}
    \caption{nBack - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=\linewidth]{example-image-a}
    \caption{nBack Negative}
  \end{subfigure}   
  \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-abcd-nback.png}
        \caption{nBack 3d Brain}
  \end{subfigure}
\caption{Top $10\%$ of the selected edges from CPM model on the resting state of both datasets. The red and blue lines are positive and negative edges, respectively. }
\label{fig:circle-plot}
\end{figure}

==> results/abcd-top5roi.tex <==
\begin{figure}[H]
     \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 1\textwidth]{imgs/abcd-top5roi.png}
         \caption{Rest}
     \end{subfigure}
      \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 0.99\textwidth]{imgs/abcd-top5roi-t1.png}
         \caption{MID}
     \end{subfigure}     
      \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 0.99\textwidth]{imgs/abcd-top5roi-t2.png}
         \caption{nBack}
     \end{subfigure}
     \begin{subfigure}[t]{0.11\textwidth}
         \vspace{-3.8cm}
         \includegraphics[width = .99\textwidth]{imgs/top5roi-legend.png}
    \end{subfigure}
    \caption{Functional Network Distributions for the largest five subunits defined by SEC(400) atlas}
    \label{fig:abcd-top5roi}
\end{figure}




==> results/hcp-cpm.tex <==
\begin{figure}[H]
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         %\includegraphics[width=0.36\textwidth]{imgs/HCP-actual-predicted-Rest.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-positive-Rest.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-negative-Rest.png}
         \caption{Rest}
     \end{subfigure}
     %\hfill
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         %\includegraphics[width=0.36\textwidth]{imgs/HCP-actual-predicted-MID.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-positive-Language.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-negative-Language.png}
         \caption{Language}
     \end{subfigure}
    % \hfill
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
         %\includegraphics[width=0.36\textwidth]{imgs/HCP-actual-predicted-nBack.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-positive-Emotion.png}
         \includegraphics[width=0.8\textwidth]{imgs/HCP-heatmap-negative-Emotion.png}
         \caption{Emotion}
     \end{subfigure}
    \caption{Heatmap of the top $20\%$ selected edges with the highest absolute value of coefficient from CPM based on SEC(400) parcellation with HCP data. The top row and bottom row visualized the positive and negative edges, and the left, middle and right column corresponds to Rest, Language and Emotion respectively. The functional networks in the plots corresponds to: 1. medial frontal, 2. fronto parietal, 3. default mode, 4. motor, 5. visual I, 6. visual II, 7. visual association, 8. limbic,  9. basal ganglia, and 10. cerebellum. }
    \label{fig:hcp-cpm-plots}
\end{figure}




==> results/hcp-parcellation-plots.tex <==
% \begin{figure}[H]
%     \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \caption{\textcolor{red}{SEK-200 (Rest)}}
%      \end{subfigure}
%      \vfill
          
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \caption{\textcolor{red}{SEK-200 (MID)}}
%      \end{subfigure}
%      \vfill
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-language.png}
%          \caption{\textcolor{red}{SEK-200 (Language)}}
%      \end{subfigure}    
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \caption{SEK-400 (Rest)}
%      \end{subfigure}
%      \vfill
          
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \caption{SEK-400 (MID)}
%      \end{subfigure}
%      \vfill
     
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \includegraphics[width=0.49\textwidth]{imgs/hcp-SEK-rest.png}
%          \caption{SEK-400 (Language)}
%      \end{subfigure}    

%     \caption{Whole brain parcellation plots visualized with BioImage Suite on HCP.}
%     \label{fig:hcp-parcellation-plots}
% \end{figure}


\begin{table}[!ht]
  \centering
  \begin{tabular}{  m{1cm} | c | c }
    \hline
    \hline
     & SBP(200) & SBP(400) \\
    %SEK & Task & Parcellation 
    \hline
    Rest 
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/hcp-SEK-rest.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-rest.png}
    \end{minipage}
    \\ \hline
    Language
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC200-ABCD-MID.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-MID.png}
    \end{minipage}
    \\ \hline
    Emotion 
    &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC200-ABCD-nBack.png}
    \end{minipage}
     &
    \begin{minipage}{.45\textwidth}
      \includegraphics[width=0.95\textwidth]{imgs/SEC400-ABCD-nBack.png}
    \end{minipage}
    \\ \hline
    \hline
  \end{tabular}
  \caption{Brain maps generated with SBP(200) and SBP(400) based on HCP dataset.}\label{tab:hcp-parc-plots}
\end{table}



==> results/hcp-sek400-ringplots.tex <==
\begin{figure}[H]
% rest
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Rest - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Rest Negative}
  \end{subfigure}   
  \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-hcp-rest.png}
        \caption{Rest 3d Brain}
  \end{subfigure}
  \vfill
%Emotion
\begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Emotion - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Emotion Negative}
  \end{subfigure}   
\begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-hcp-emotion.png}
        \caption{Emotion 3d Brain}
  \end{subfigure}
  \vfill
%NBACK
\begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Language - positive}
  \end{subfigure}   
  \hfill
  \begin{subfigure}{0.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{example-image-b.png}
    \caption{Language Negative}
  \end{subfigure}   
  \begin{subfigure}{0.33\textwidth}
        \includegraphics[width=\textwidth]{imgs/connectome-sek400-hcp-language.png}
        \caption{Language 3d Brain}
  \end{subfigure}
  \vfill
% Legend 
 % \begin{subfigure}{0.1\textwidth}
 %    \centering
 %    \includegraphics[width=.9\linewidth]{imgs/connectivity-annotation.png}
 %  \end{subfigure}  
\caption{Top $10\%$ of the selected edges from CPM model on the resting state of both datasets. The red and blue lines are positive and negative edges, respectively. }
\label{fig:hcp-circle-plot}
\end{figure}

==> results/hcp-top5roi.tex <==
\begin{figure}[H]
     \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 1\textwidth]{imgs/hcp-top5roi.png}
         \caption{Rest}
     \end{subfigure}
      \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 0.99\textwidth]{imgs/hcp-top5roi-t1.png}
         \caption{Language}
     \end{subfigure}     
      \begin{subfigure}[t]{0.29\textwidth}
         \centering
         \includegraphics[width = 0.99\textwidth]{imgs/hcp-top5roi-t2.png}
         \caption{Emotion}
     \end{subfigure}
     \begin{subfigure}[t]{0.11\textwidth}
         \vspace{-3.8cm}
         \includegraphics[width = .99\textwidth]{imgs/top5roi-legend.png}
    \end{subfigure}
    \caption{Functional Network Distributions for the largest five subunits defined by SEC(400) atlas.}
    \label{fig:hcp-top5roi}
\end{figure}

